CoMeT: Count-Min-Sketch-based Row Tracking to Mitigate RowHammer at Low Cost

We propose a new RowHammer mitigation mechanism, CoMeT, that prevents RowHammer bitflips with low area, performance, and energy costs in DRAM-based systems at very low RowHammer thresholds. The key idea of CoMeT is to use low-cost and scalable hash-based counters to track DRAM row activations. CoMeT uses the Count-Min Sketch technique that maps each DRAM row to a group of counters, as uniquely as possible, using multiple hash functions. When a DRAM row is activated, CoMeT increments the counters mapped to that DRAM row. Because the mapping from DRAM rows to counters is not completely unique, activating one row can increment one or more counters mapped to another row. Thus, CoMeT may overestimate, but never underestimates, a DRAM row's activation count. This property of CoMeT allows it to securely prevent RowHammer bitflips while properly configuring its hash functions reduces overestimations. As a result, CoMeT 1) implements substantially fewer counters than the number of DRAM rows in a DRAM bank and 2) does not significantly overestimate a DRAM row's activation count. Our comprehensive evaluations show that CoMeT prevents RowHammer bitflips with an average performance overhead of only 4.01% across 61 benign single-core workloads for a very low RowHammer threshold of 125, normalized to a system with no RowHammer mitigation. CoMeT achieves a good trade-off between performance, energy, and area overheads. Compared to the best-performing state-of-the-art mitigation, CoMeT requires 74.2x less area overhead at the RowHammer threshold 125 and incurs a small performance overhead on average for all RowHammer thresholds. Compared to the best-performing low-area-cost mechanism, at a very low RowHammer threshold of 125, CoMeT improves performance by up to 39.1% while incurring a similar area overhead. CoMeT is openly and freely available at https://github.com/CMU-SAFARI/CoMeT.

==> hpca-template.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% -- DO NOT MODIFY -- %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\author{
  \ifdefined\hpcacameraready
    \IEEEauthorblockN{\hpcaauthors{}}
      \IEEEauthorblockA{
        \hpcaaffiliation{} \\
        \hpcaemail{}
      }
  \else
    \IEEEauthorblockN{\normalsize{HPCA \hpcayear{} Submission
      \textbf{\#\hpcasubmissionnumber{}}} \\
      \IEEEauthorblockA{
        Confidential Draft \\
        Do NOT Distribute!!
      }
    }
  \fi 
}

% Heading and footer for title page
\fancypagestyle{camerareadyfirstpage}{%
  \fancyhead{}
  \renewcommand{\headrulewidth}{0pt}
  \fancyhead[C]{
    \ifdefined\aeopen
    \parbox[][12mm][t]{13.5cm}{\hpcayear{} IEEE International Symposium on High-Performance Computer Architecture (HPCA)}    
    \else
      \ifdefined\aereviewed
      \parbox[][12mm][t]{13.5cm}{\hpcayear{} IEEE International Symposium on High-Performance Computer Architecture (HPCA)}
      \else
      \ifdefined\aereproduced
      \parbox[][12mm][t]{13.5cm}{\hpcayear{} IEEE International Symposium on High-Performance Computer Architecture (HPCA)}
      \else
      \parbox[][0mm][t]{13.5cm}{\hpcayear{} IEEE International Symposium on High-Performance Computer Architecture (HPCA)}
    \fi 
    \fi 
    \fi 
    \ifdefined\aeopen 
      \includegraphics[width=12mm,height=12mm]{ae-badges/open-research-objects.pdf}
    \fi 
    \ifdefined\aereviewed
      \includegraphics[width=12mm,height=12mm]{ae-badges/research-objects-reviewed.pdf}
    \fi 
    \ifdefined\aereproduced
      \includegraphics[width=12mm,height=12mm]{ae-badges/results-reproduced.pdf}
    \fi
  }
  %\fancyfoot[L]{\hpcapubid{} \copyright \hpcayear{} IEEE}
  \fancyfoot[C]{}
}
% Heading and footer for remaining pages
\fancyhead{}
\renewcommand{\headrulewidth}{0pt}
%\fancyhead[C]{\hpcayear{} IEEE International Symposium on
% High-Performance Computer Architecture (HPCA)}


\begin{document}
\maketitle

%Enables the camera ready header and footer
\ifdefined\hpcacameraready 
  \thispagestyle{camerareadyfirstpage}
  \pagestyle{empty}
\else
  \thispagestyle{plain}
  \pagestyle{plain}
\fi

\newcommand{\hpcaheight}{0mm}
\ifdefined\eaopen
\renewcommand{\hpcaheight}{12mm}
\fi
  

